Querying Large Language Models with SQL

In many use-cases, information is stored in text but not available in structured data. However, extracting data from natural language text to precisely fit a schema, and thus enable querying, is a challenging task. With the rise of pre-trained Large Language Models (LLMs), there is now an effective solution to store and use information extracted from massive corpora of text documents. Thus, we envision the use of SQL queries to cover a broad range of data that is not captured by traditional databases by tapping the information in LLMs. To ground this vision, we present Galois, a prototype based on a traditional database architecture, but with new physical operators for querying the underlying LLM. The main idea is to execute some operators of the the query plan with prompts that retrieve data from the LLM. For a large class of SQL queries, querying LLMs returns well structured relations, with encouraging qualitative results. Preliminary experimental results make pre-trained LLMs a promising addition to the field of database systems, introducing a new direction for hybrid query processing. However, we pinpoint several research challenges that must be addressed to build a DBMS that exploits LLMs. While some of these challenges necessitate integrating concepts from the NLP literature, others offer novel research avenues for the DB community.

==> response.tex <==
\renewcommand{\ni}{\noindent}
\newcommand{\stab}{\vspace{1.2ex}\noindent}
\newcommand{\etitle}[1]{\vspace{0.8ex}\noindent{\underline{\em #1}}}
\newcommand{\red}[1]{\textcolor{red}{#1}}

%cover letter (up to 4 pages)
\twocolumn [\begin{center}\huge{\textbf{EDBT 2024 Paper 61: Response to Reviewer Comments for \\{\em [Vision Paper] Querying Large Language Models with SQL}}}\end{center}\vspace{8ex}]

\ni {\bf{\em Dear EDBT Reviewers:}}

\stab
We thank the reviewers for their insightful comments, based on which we have made significant changes to improve the paper. The new material in the paper is highlighted in \rev{blue}. We start with a description of our major changes according to the metareview instructions.

%METAREVIEW
%This vision paper discusses a timely topic, combining Large Language Models (LLMs) with SQL queries to extract information from unstructured text. The reviewers would like to see more results, explanations and details. The reviewers would like to give the authors a chance to revise. Also, the final decision would be dependent upon how well the concerns are addressed in the revision. Please refer to the reviewers' comments for detail.
% 3. Summary of Items For Revision
% 1) It needs to discuss more the functional architecture for an LLM-SQL query engine, the motivation given the other possible approaches, and emphasizes differences from previous research and highlight transformative implications of LLMs

% 2) More discussion on textual prompts, prompt construction, and hallucinations.

% 3) The experimental studies. There are some concerns on the experimental studies. It is expected to have some experimental studies to allow a good understanding of the results and limitations.
 
\stab
{\bf C1: Architecture.} We have rewritten the paper to emphasize the general vision and present our initial work as one possible solution in the \textit{DB-first} direction. 
%See also response to R1(O2).

\stab
{\bf C2: Discussions.} We rewrote the sections involving some challenges (including hallucinations) and possible solutions with textual prompt engineering.
%See also response to R2(O1).

\stab
{\bf C3: Experiments.} We extended the experimental section and now emphasize the lesson taken from our initial implementation and the limitations of such approach. 
%See also responses to R2(O2), R2(O3), R2(O4), R3(O1).


\stab
We also addressed all the minor issues and introduced clarifications in terms of presentation. 

\stab
While we did our best effort to implement the suggestions from the reviewers, we were not able to expand a short vision paper to include all the details and experiments that would be expected in a full research paper. We believe our submission is aligned with the expectations for a vision paper as detailed in the EDBT 2024 CFP:

``\textit{Vision submissions describe emerging areas of research or new applications of data management technology. Papers in this track are not required to
present research results. Rather, they may articulate a vision for future
research in an important new area, identify challenging technical problems
to be addressed, and explain potential technical or social impact.}'' (\url{https://dastlab.github.io/edbticdt2024/?contents=EDBT_CFP.html}).




%\vspace{4ex}
\section*{Responses to the Comments of Reviewer 2.}

%IMPORTANT: I would recommend strengthening the argument for applications even though the work is interesting without downstream applications. I would also recommend making sure your argument on using TENET for each domain is consistent with the results that show that TNLI models trained thus can generalize nicely out-of-domain.
%IMPORTANT ++++++++++++++++++++++++++++++++++++++

%\vspace{0.8ex}
\etitle{R2(D1).}
{\em D1: I don't understand the analysis of the cardinality (function f). First, what is the definition of $R_G$ ($R_G=R_M?$)? Second, if the formula is f=2*|$R_D$|/|$R_D$|+|$R_M$|, the interval for f is ]0.2]. How do you get the values in Table 1?
}

\stab
{\bf [A]}
Sorry for the confusion, indeed $R_G=R_M$ (\system's output when executed on LLM $M$). We fixed the typo in the revision. 

We now clarify that the interval for $f$ is [0,2] and best result occurs when $R_D==R_M$ (f=1). Consider expected relation $R_D$ with size (3,2), i.e. 3 tuples and 2 columns. Assume \system produced $R_M$ = (1,2). We compare the number of tuples as the columns are constrained by the query plan. In this case, f = |2*3| / (3+1) = 6/4 = 1.5.  We then average through the queries and compute 1-f (values in Table 1).



\vspace{0.8ex}
\etitle{R2(D2).}
{\em How do you measure precision? Is Spider complete with respect to the knowledge of ChatGPT? What exactly are the queries you ask?}

\stab
{\bf [A]} We now better clarify that accuracy (Table 2) is computed as cell value matches between the result returned by a method and the same query executed on the original relational data in the Spider database (ground truth).

We now clearly state that some questions in Spider are dependent on a proprietary dataset, e.g., ``What are the first, middle, and last names, along with the ids, of all students who enrolled in 2 degree programs in one semester?”. For this reason we select datasets and questions that are on generic topics covered by public LLMs (e.g., ``What are the names of all the countries that became independent after 1950?”). 


\vspace{0.8ex}
\etitle{R2(D3).}
{\em The correctness for join is 0? This is not very encouraging for the motivation to use SQL?}

\stab
{\bf [A]}
We report such negative results for our prototype because we believe it is useful to show that the problem is not trivial. Notice that also the NL prompt based solution fails for this subclass. The challenge in querying with joins motivates further research, which is one of the goals of our vision. We now state this in the revision.



\vspace{0.8ex}
\etitle{R2(D4).}
{\em Textual prompts: The automatic generation of precise textual prompts for given attribute labels is critical to the proposed approach. You mention fine-tuning and using predefined embeddings for attribute types as a possible solution. Could you provide some more details on how these solutions could be integrated into the query engine?
}

\stab
{\bf [A]}
We have added details in the revision (Section 6), including fine-tuning the model according to human-preferences, e.g., RLHF, %(https://arxiv.org/abs/2204.05862)(https://direct.mit.edu/tacl/article/doi/10.1162/tacl_a_00279/43493/Trick-Me-If-You-Can-Human-in-the-Loop-Generation) 
and using pre-defined embeddings as a sort of prior to the model when generating output, e.g., Type Embeddings. % (https://aclanthology.org/2022.findings-emnlp.336/)




\vspace{0.8ex}
\etitle{R2(D5).}
{\em Hallucinations: You also mention the problem of hallucinations, which is a major issue when using generative language models to answer questions. Again, it would be interesting to get some more information on how the methods you mention could be integrated into the query engine.
}

\stab
{\bf [A]}
We have extended the discussion on detecting whether the model is hallucinating in Section 4 by methods such as having the generated output critiqued by another model %(https://arxiv.org/pdf/2303.11366.pdf) (https://arxiv.org/pdf/2305.15852.pdf) 
or by augmenting the LLMs with external information. % (https://dl.acm.org/doi/10.1145/3571730).



\section*{Responses to the Comments of Reviewer 3.}


\etitle{R3(D1).}
{\em I believe that this work should underscore the fundamental differences between their approach and previous research, beyond the realm of specific design aspects. There has been considerable exploration in the field regarding the integration of NLP neural networks with databases prior to the prevalence of LLMs. It is important to provide a more pronounced emphasis on the transformative implications of the rapid advancement of LLMs in the present context.

}

\stab
{\bf [A]}
Previous approaches to extract structured data from text rely on ML models that require expensive training data.
We now better clarify across the paper that the approach of querying LLMs enables  the ability to query documents without human pre-processing. 

%As one important related research direction, we added a discussion about tabular language models. %(https://direct.mit.edu/tacl/article/doi/10.1162/tacl_a_00544/115239). However, this topic is different from Galois, as the goal here is not to incorporate tabular structure, but instead to query with SQL existing LLMs created from any corpus.

In terms of transformative implications, we rewrote the `Architecture' part in Section 6 to report evidence that an LLM-first solution could not replace DBMSs even in a simple read-only setting, because of multiple issues. Even if LLMs' progress continues with the current pace, legal and economic hurdles (e.g., the need for formal guarantees in transactions) are likely to limit the impact of LLM-first approaches in data management tasks.


\vspace{0.8ex}
\etitle{R3(D2).}
{\em The paper presents experimental validation of the proposed method; however, the analysis of the experimental results is relatively limited. It would greatly enhance the paper if the experimental section provided a more in-depth analysis of the results, showcased a broader range of experimental outcomes.}



\stab
{\bf [A]}
We agree that more experiments and details would be interesting to report, but we are limited by the six-page constraint for papers in the Vision track. At the same time, we show the potential of a DB-first approach with an early prototype and we are not claiming that it is a solid system. Our goal with the experiments is to show potential and motivate further research in this direction. 


\vspace{0.8ex}
\etitle{R3(D3).}
{\em The paper lacks a comprehensive showcase of their presented prototype, and the description provided is somewhat superficial.}

\stab
{\bf [A]}
We have added more details about the prototype in Section 5 (Implementation) and refer the readers to the Git repository for %an extended version for 
%a more detailed presentation of 
implementation and datasets.  %and additional experimental results.


\vspace{0.8ex}
\etitle{R3(D4).}
{\em I believe it would be valuable for the authors to increase the mention and discussion of prompt engineering in their paper. Prompt engineering impacts the practical performance of LLMs, and the proposed approach may rely on prompt construction.
}


\stab
{\bf [A]}
Our initial prototype is intentionally very lightweight in terms of prompt engineering. This is a topic in rapid evolution 
%(https://arxiv.org/pdf/2107.13586.pdf) 
and we are not claiming contributions in this aspect. On the contrary, DB-first approaches directly exploit new results in prompt engineering, as those could be easily plugged in step 2 of the workflow (Section 4). We now clarify this point in the revised text.

We have also introduced a new baseline method with a more refined prompt for questions answering.


\section*{Responses to the Comments of Reviewer 4.}

%\vspace{0.8ex}
\etitle{R4(D1).}
{\em 
%The presented vision is cool, interesting, and unconventional, however, the authors should have done a better job at motivating its need. The primary use-case presented in the introduction is around information extraction (IE) from unstructured data, and how a SQL-like interface to LLMs aid in addressing this fundamental problem. However, it is unclear to me whether this is the correct use-case. Specifically, 
[...] why can't IE systems based on LLMs extract the required structured information from unstructured data, be stored in a traditional DBMS, and then be queried using SQL? After all, as per the vision, SQL queries first extract structured data in the form of tuples/relations by prompting LLMs relations, then what is the problem with the existing two-phase paradigm of IE followed by querying structured information?

%Update after reading author feedback: Thanks for the clarification, but I don't think the authors clearly understood my point. 
[...]
%I disagree with the authors' claim that the materialization direction (obtain relations and store in DBMS) would be enabled only by the approach proposed in this paper. 
%My main point in the above comment was that 
there should be specialized IE tools (leveraging either LLMs or any other technology) with the sole objective of extracting relations from unstructured text, which can then be simply queried via SQL. In that case, there is no clear need for the paradigm that the authors propose in this work. My expectation from the authors is that they should clearly discuss the pros and cons of both the paradigms and then clearly articulate what could be solved by their proposed paradigm which cannot be done using the simpler two-phase materialization approach.}
\stab

{\bf [A]}
Thanks for the clarification, we did not get the point correctly in our feedback response.
We now mention in the revised text across the paper the two main shortcomings in the traditional materialization approach (obtain structured data and store in DBMS). 

First, such approaches require training data and human work, even when using tools, such as Snorkel, that help users in annotating data. Out-of-box NLP solutions work well only for an handful of entities (e.g., Location and People) in name entity recognition. 

Second, assuming training data is provided, only binary relations can be effectively extracted - results for n-ary relations are not directly usable.

In contrast, LLMs and prompts enable the extraction of structured data without human annotations. The benefit of the DB-first approach is that the prompts are automatically generated, thanks to the logical plan.

Another important aspect is that hybrid querying enables optimizations across the operators executed over the LLM and the DB. This is not possible with the materialization approach in a waterfall fashion. 
%However, we stress that this would be enabled by the approach that we are proposing: for complex IE tasks (see next point), the creation of the relation requires to run the SQL query on the LLM, which is part of the vision.




\vspace{0.8ex}
\etitle{R4(D2).}
{\em 
%Although the authors discuss this aspect a bit, but it is still not clear to me what is the fundamental difference between the proposed paradigm of using SQL to query LLMs and prompting. While the authors cite certain limitations of NL prompts, i.e., they lack precision, among others, I believe such claims are not entirely well-founded. NL prompts can be easily made more structured and well-defined, e.g., AutoGPT, GPTEngineer, etc., and even lead to outputs in structured format, such as code, json, markdown, etc. Thus, the claim that we need a SQL like interface is stretching it a bit too far. Moreover, NL prompts are much more user friendly than using a declarative programming language such as SQL. So, if using NL is enough, there should be a justified reason to increase the complexity and reduce the user friendliness of querying LLMs. Eventually, the implementation of the prototype is realized using some form of chain-of-thought prompting, thus, I urge the authors to clearly articulate the differences from prompting.
%Update after reading author feedback: The claims that "logical plan is an excellent way to break complex tasks in smaller ones" and "when the NL question is complex or requires combining multiple elements, a declarative programming language such as SQL leads to more precise specifications" are spot on, but 
[...]
this still requires the user to come up with a SQL query, which should be promptly acknowledged early in the paper. On the other hand, most examples that the authors use in their paper can be easily decomposed into multiple tasks by humans using NL prompts. IMHO, the secret sauce is chain-of-thought prompting, and I would encourage the authors to discuss the pros and cons of their approach (SQL followed by a logical plan) and contrast it with the pros and cons of an approach that uses well-engineered chain-of-thought NL prompts.
}

\stab
{\bf [A]}
Thanks again for the clarification after the feedback. In the revised text, we now clarify three aspects highlighted by the reviewer.

First, we state early in the paper that the SQL script is user provided. 

Second, we highlight across the paper that a clear advantage of the DB-first approach is the automatic generation of chain-of-thought prompts. Moreover, we now stress that the ability to combine in one query plan operators over traditional storage and LLMs is a vision that go beyond the scope of chain-of-thought. For example, a novel query optimizer may be able to recognize when the execution of the (more expensive) LLM is needed at runtime.

Third, we added remarks on the pros and cons of querying LLM vs using well-engineered chain-of-thought NL prompts. %While the latter may lead to better results, 
We argue that the main benefit of the vision is the ability to obtain such elaborate chain of prompts automatically (see also R4(D1)).

%We show that the logical plan is an excellent way to break complex tasks in smaller ones, which is a winning paradigm in LLMs. This is a natural and elegant approach to break down a complex SQL prompt in simpler steps, without using generic solutions like AutoGPT or GPTEngineer. For example, “What is the average male life expectancy in the countries where English is not the official language?“ is easier to answer through its decomposition. In Galois, the chain-of-thought prompting is obtained automatically by exploiting the logical plan, with multiple benefits, such as the production of relations (by construction) and the enabling of optimization to reduce the overall execution cost.

%b) We agree that NL prompts are more user friendly for simple queries in use cases such as chatbots with end users. However, when the NL question is complex or requires  combining multiple elements, a declarative programming language such as SQL leads to more precise specifications. For example the question “Return the list of companies that have higher revenues but lower tax rates than other companies, with the first group constrained to EU countries, while the second group can be from any country, without comparing companies from the same country”. Also, for a use case where both a DB and a LLM are needed to answer a question, our approach enables hybrid querying with SQL, e.g., query q in Sec. 1.  



\vspace{0.8ex}
\etitle{R4(D3).}
{\em Using the NL question t as a prompt to extract the answer is an overly simple baseline, and therefore may not present a fair comparison with GALOIS. I would urge the authors to implement chain-of-thought prompts based on the NL question t, and then use such a modified prompt to query the LLMs, which would provide a stronger and fairer baseline comparison for the proposed system.

%Update after reading author feedback: "We can add experiments with examples given as few shots and explicitly adding to the prompt 'Answer the question step by step'". This is a good start for an improved baseline, but I don't think this would be enough. 
[...]
You should prepare chain-of-thought NL prompt templates that poses the query to the LLM by breaking down the tasks into simpler units. Note that I am not suggesting to create a decomposition for each query manually, but you should come up with a decomposition that is possible programmatically and can be automated. For example, you can even ask another LLM model to break down the full NL query into multiple small tasks, which would be then input to the model that answers these decomposed tasks. IMHO, contextualizing your findings with such an improved baseline is super important to establish the need for your visionary research.}

\stab
{\bf [A]}
We have added a new baseline based on this suggestion for question answering. The new prompt (NL+CoT) contains an example of a chain-of-thought similar to our logical plan execution, followed by instruction to reason step by step.
The results show a slight degradation in results, compared to the original NL questions. While the CoT produces a valid chain of thought, it abstains from providing concrete numbers for, as an example, the surface area for each country in the Caribbean Region mentioning that such numbers can be obtained from reliable resources. Thus, the CoT approach does not answer the question of the total sum of such surface areas. The QA approach without CoT turns out to be more factual in the responses, i.e., directly provides the answer of the total surface area. 

Our approach derives a chain of prompts
from a SQL script, but how to obtain a similar decomposition automatically from a question in NL is an open problem.  We now state this direction of research in Section 5.




\vspace{0.8ex}
\etitle{R4(D4).}
{\em 
Automatically detecting whether the model is hallucinating should also be a module in a system such as GALOIS. I would appreciate if the authors can include a discussion around this aspect in Section-6.

LLMs can be asked to utter an explanation supporting their output, which often includes a description of the thought process and the source of information. Thus, the claim that LLMs do not expose the sources with the results may not be entirely true. This completely depends on how they are prompted and what they are asked to output.
}

\stab
{\bf [A]} We have extended the discussion on detecting hallucinations in Section 4, including having the generated output critiqued by another model %(https://arxiv.org/pdf/2303.11366.pdf) (https://arxiv.org/pdf/2305.15852.pdf) 
and augmenting the LLMs with external information. % 

We added a clarification on the ability of LLMs to produce explanations in Section 6.


\section*{Responses to the Comments of Reviewer 5.}

\etitle{R5(D1).}
{\em 
First, the training of LLMs is limited to training data and has its own accuracy problem.

To query LLMs, there is another important issue about the accuracy of the answers provided by LLMs. LLMs may provide wrong answers, but still give fake evidence.

The proposed solution lacks of some verification method about the query results.

}

\stab
{\bf [A]} 
As we discuss in Section 6, training data raise several problems, but this aspect is getting more and more attention with promising new results. We have added two recent works that have been released since our submission to EDBT that address the quality of the training data. %(https://arxiv.org/abs/2306.11644,  https://arxiv.org/abs/2306.01116).

We have extended our discussion for model hallucinations, as detailed in the response to R2(D5).

For the verification, we used manual evaluation for the results reported in Table 2. An accurate metric for comparing the returned results is an open problem that we now clarify in the revised version of the paper.



\vspace{0.8ex}
\etitle{R5(D2).}
{\em There is one concern why authors consider using SQL to query LLMs, rather than natural languages or query graphs.

When using SQLs, it assumes that data schema has been designed. So it is not clear how to define this data schema from text data.

If this data schema is available, then it comes back to the problem of extracting values of attributes in the schema. Please provide the reasons why the LLMs can provide more accurate answers than existing data extraction methods.
}

\stab
{\bf [A]} 
Please see point R4(D1) and R4(D2) for the motivation of using SQL rather than NL questions.

For query graphs, we believe our vision can be extended to SPARQL, but we are not aware of solutions to query LLMs with graph patterns.

We let users come up with their schema, which we use to derive the query plan. We discuss as open problem the setting where the query is defined without providing a schema (Section 6).

For the last point, please see the response to R4(D2).
We allow an arbitrary schema for querying the LLM. It is not clear how to automatically populate such schema with tuples extracted from raw text without a significant manual effort in writing scripts (or in creating training data).
%- standard NLP tools can get entities and few binary relationships out of the box only for very common types, such as City, Person, Company.

%In data extraction tasks, LLMs provide more accurate answers than existing methods because of the breakthrough in the last few years in NLP language understanding with transformers and self supervised learning on large corpora.


\vspace{0.8ex}
\etitle{R5(D3).}
{\em Please discuss how to convert SQLs into the input of LLMs.
}


\stab
{\bf [A]} 
\system automatically converts SQLs logical operators as NL prompts to be executed on the LLM - we revised Section 1 and Section 4 to clarify this point. 

\vspace{0.8ex}
\etitle{R5(D4).}
{\em 
As mentioned in Section 1, there is a requirement "the same SQL script should return the same answer when executed on any pre-trained LLM that exposes textual prompts". It is not clear how to achieve this goal.
}

\stab
{\bf [A]} 
We presented as a requirement that an SQL script should return the same answer when executed on different LLMs, but we now reposition this aspect as a research challenge in our vision (Section 6, Portability). 



\vspace{5ex}
\noindent {\large\em Yours sincerely,}

\vspace{1.8ex}
{\large\em The authors}

%\balance
\clearpage

